On the Generalization Effects of Linear Transformations in Data Augmentation

Data augmentation is a powerful technique to improve performance in applications such as image and text classification tasks. Yet, there is little rigorous understanding of why and how various augmentations work. In this work, we consider a family of linear transformations and study their effects on the ridge estimator in an over-parametrized linear regression setting. First, we show that transformations that preserve the labels of the data can improve estimation by enlarging the span of the training data. Second, we show that transformations that mix data can improve estimation by playing a regularization effect. Finally, we validate our theoretical insights on MNIST. Based on the insights, we propose an augmentation scheme that searches over the space of transformations by how uncertain the model is about the transformed data. We validate our proposed scheme on image and text datasets. For example, our method outperforms random sampling methods by 1.24% on CIFAR-100 using Wide-ResNet-28-10. Furthermore, we achieve comparable accuracy to the SoTA Adversarial AutoAugment on CIFAR-10, CIFAR-100, SVHN, and ImageNet datasets.

==> compile_log <==
This is pdfTeX, Version 3.14159265-2.6-1.40.16 (TeX Live 2015) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./main_two_col.tex
LaTeX2e <2015/01/01>
Babel <3.9l> and hyphenation patterns for 79 languages loaded.
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/article.cls
Document Class: article 2014/09/29 v1.4h Standard LaTeX document class
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/size10.clo))
(/usr/local/texlive/2015/texmf-dist/tex/latex/microtype/microtype.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/microtype/microtype-pdftex.def)
(/usr/local/texlive/2015/texmf-dist/tex/latex/microtype/microtype.cfg))
(/usr/local/texlive/2015/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/caption/caption3.sty)))
(/usr/local/texlive/2015/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/graphics.cfg)
(/usr/local/texlive/2015/texmf-dist/tex/latex/pdftex-def/pdftex.def
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/infwarerr.sty)
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/ltxcmds.sty))))
(/usr/local/texlive/2015/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/tools/xspace.sty)
(./macro_math.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/amscls/amsthm.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsfonts/amssymb.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/jknapltx/mathrsfs.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/color.cfg))
(/usr/local/texlive/2015/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/bbm-macros/bbm.sty))
(./icml2020.sty (/usr/local/texlive/2015/texmf-dist/tex/latex/psnfss/times.sty)
 (./fancyhdr.sty) (./algorithm.sty
Document Style `algorithm' - floating environment
(/usr/local/texlive/2015/texmf-dist/tex/latex/float/float.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/base/ifthen.sty))
(./algorithmic.sty
Document Style `algorithmic' - environment
(/usr/local/texlive/2015/texmf-dist/tex/latex/tools/calc.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/natbib/natbib.sty)
(/usr/local/texlive/2015/texmf-dist/tex/latex/eso-pic/eso-pic.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/atbegshi.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/ifpdf.sty)))
(/usr/local/texlive/2015/texmf-dist/tex/latex/forloop/forloop.sty))
(./main_two_col.aux)
(/usr/local/texlive/2015/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
(/usr/local/texlive/2015/texmf-dist/tex/latex/microtype/mt-ptm.cfg)
(/usr/local/texlive/2015/texmf-dist/tex/context/base/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/pdftexcmds.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/ifluatex.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/grfext.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/kvdefinekeys.sty))
(/usr/local/texlive/2015/texmf-dist/tex/latex/oberdiek/kvoptions.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/kvsetkeys.sty
(/usr/local/texlive/2015/texmf-dist/tex/generic/oberdiek/etexcmds.sty)))
(/usr/local/texlive/2015/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2015/texmf-dist/tex/latex/microtype/mt-cmr.cfg)
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2015/texmf-dist/tex/latex/microtype/mt-msa.cfg)
(/usr/local/texlive/2015/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2015/texmf-dist/tex/latex/microtype/mt-msb.cfg)
(/usr/local/texlive/2015/texmf-dist/tex/latex/jknapltx/ursfs.fd)
(/usr/local/texlive/2015/texmf-dist/tex/latex/psnfss/omlptm.fd)
(/usr/local/texlive/2015/texmf-dist/tex/latex/psnfss/omsptm.fd) (./intro.tex
Overfull \hbox (2.94391pt too wide) in paragraph at lines 125--125
[]\OT1/ptm/m/n/10 (-20) Transformations| 

Overfull \hbox (2.19423pt too wide) in paragraph at lines 123--135
 [][] 
<figures/pyramidnet_aug_shift.pdf, id=1, 1405.25pt x 552.0625pt>
<use figures/pyramidnet_aug_shift.pdf>
Underfull \vbox (badness 10000) has occurred while \output is active [1{/usr/lo
cal/texlive/2015/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
Underfull \vbox (badness 10000) has occurred while \output is active)
(./modeling.tex
Underfull \vbox (badness 10000) has occurred while \output is active [2 <./figu
res/pyramidnet_aug_shift.pdf>]) (./theory.tex [3] [4]) (./aug_analysis.tex
<./figures/mnist_instability.pdf, id=52, 803.0pt x 652.4375pt>
<use ./figures/mnist_instability.pdf>
<./figures/composition.pdf, id=53, 361.0861pt x 254.73608pt>
<use ./figures/composition.pdf>
(/usr/local/texlive/2015/texmf-dist/tex/latex/bbm-macros/ubbm.fd) [5]
Underfull \vbox (badness 10000) has occurred while \output is active)
(./experiments.tex
Underfull \vbox (badness 10000) has occurred while \output is active [6 <./figu
res/mnist_instability.pdf> <./figures/composition.pdf>]

LaTeX Warning: `h' float specifier changed to `ht'.


LaTeX Warning: `h' float specifier changed to `ht'.


Underfull \vbox (badness 10000) has occurred while \output is active
Underfull \hbox (badness 1776) in paragraph at lines 146--155
[]\OT1/ptm/b/n/10 Improving train-ing ef-fi-ciency over Ad-ver-sar-ial Au-

Underfull \vbox (badness 10000) has occurred while \output is active [7]

LaTeX Font Warning: Command \small invalid in math mode on input line 245.


LaTeX Font Warning: Command \small invalid in math mode on input line 251.


LaTeX Font Warning: Command \small invalid in math mode on input line 252.


Underfull \hbox (badness 1681) in paragraph at lines 251--253
[]\OT1/ptm/m/it/10 (+20) Comparison meth-ods\OT1/ptm/m/n/10 (+20) . We com-pare
 with pre-BERT

LaTeX Font Warning: Command \small invalid in math mode on input line 265.


LaTeX Font Warning: Command \small invalid in math mode on input line 271.


LaTeX Font Warning: Command \small invalid in math mode on input line 271.


Underfull \vbox (badness 1248) has occurred while \output is active)
(./related.tex
Underfull \vbox (badness 10000) has occurred while \output is active [8]
Underfull \vbox (badness 10000) has occurred while \output is active)
(./main_two_col.bbl

Package balance Warning: You have called \balance in second column
(balance)                Columns might not be balanced.

[9] [10]) [11] (./appendix_theory.tex [12]
Overfull \hbox (9.39043pt too wide) in paragraph at lines 81--81
[] 
[13] [14]
Overfull \hbox (15.71051pt too wide) in paragraph at lines 202--202
[] 
[15] [16] [17] [18]) (./appendix_experiments.tex [19]

LaTeX Font Warning: Command \small invalid in math mode on input line 55.


LaTeX Font Warning: Command \small invalid in math mode on input line 110.

) (./appendix_mixup.tex

LaTeX Warning: `!h' float specifier changed to `!ht'.


Underfull \vbox (badness 10000) has occurred while \output is active [20]
<figures/cifar_margin_all.pdf, id=125, 602.25pt x 552.0625pt>
<use figures/cifar_margin_all.pdf>
<figures/cifar_margin_correct.pdf, id=126, 602.25pt x 552.0625pt>
<use figures/cifar_margin_correct.pdf>
<figures/cifar_margin_wrong.pdf, id=127, 602.25pt x 552.0625pt>
<use figures/cifar_margin_wrong.pdf>
<figures/cifar_margin_wrong_ratio.pdf, id=128, 602.25pt x 552.0625pt>
<use figures/cifar_margin_wrong_ratio.pdf>) [21 <./figures/cifar_margin_all.pdf
> <./figures/cifar_margin_correct.pdf> <./figures/cifar_margin_wrong.pdf> <./fi
gures/cifar_margin_wrong_ratio.pdf>] (./main_two_col.aux) )
(see the transcript file for additional information) </Users/hongyang/Library/t
exlive/2015/texmf-var/fonts/pk/ljfour/public/bbm/bbm10.600pk>{/usr/local/texliv
e/2015/texmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2015/texmf-di
st/fonts/type1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2015/texmf-dis
t/fonts/type1/public/amsfonts/cmextra/cmex9.pfb></usr/local/texlive/2015/texmf-
dist/fonts/type1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2015/texmf-d
ist/fonts/type1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2015/texmf-dis
t/fonts/type1/public/amsfonts/cm/cmmi6.pfb></usr/local/texlive/2015/texmf-dist/
fonts/type1/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2015/texmf-dist/fo
nts/type1/public/amsfonts/cm/cmmi9.pfb></usr/local/texlive/2015/texmf-dist/font
s/type1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2015/texmf-dist/fonts/
type1/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2015/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr6.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/
public/amsfonts/cm/cmr7.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/pub
lic/amsfonts/cm/cmr9.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/public/
amsfonts/cm/cmsy5.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/public/am
sfonts/cm/cmsy6.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/public/amsf
onts/cm/cmsy7.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/public/amsfon
ts/cm/cmsy9.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/public/amsfonts
/cm/cmti9.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/public/amsfonts/s
ymbols/msam10.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/public/amsfon
ts/symbols/msbm10.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/public/am
sfonts/symbols/msbm7.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/urw/ti
mes/utmb8a.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/urw/times/utmr8a
.pfb></usr/local/texlive/2015/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr
/local/texlive/2015/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on main_two_col.pdf (21 pages, 464800 bytes).
Transcript written on main_two_col.log.

